Semi-Blind Inference of Topologies and Dynamical Processes over Graphs

Network science provides valuable insights across numerous disciplines including sociology, biology, neuroscience and engineering. A task of major practical importance in these application domains is inferring the network structure from noisy observations at a subset of nodes. Available methods for topology inference typically assume that the process over the network is observed at all nodes. However, application-specific constraints may prevent acquiring network-wide observations. Alleviating the limited flexibility of existing approaches, this work advocates structural models for graph processes and develops novel algorithms for joint inference of the network topology and processes from partial nodal observations. Structural equation models (SEMs) and structural vector autoregressive models (SVARMs) have well-documented merits in identifying even directed topologies of complex graphs; while SEMs capture contemporaneous causal dependencies among nodes, SVARMs further account for time-lagged influences. This paper develops algorithms that iterate between inferring directed graphs that "best" fit the data, and estimating the network processes at reduced computational complexity by leveraging tools related to Kalman smoothing. To further accommodate delay-sensitive applications, an online joint inference approach is put forth that even tracks time-evolving topologies. Furthermore, conditions for identifying the network topology given partial observations are specified. It is proved that the required number of observations for unique identification reduces significantly when the network structure is sparse. Numerical tests with synthetic as well as real datasets corroborate the effectiveness of the novel approach.

==> icasspbib.tex <==
% Generated by IEEEtranS.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtranS.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{anis2016proxies}
A.~Anis, A.~Gadde, and A.~Ortega, ``Efficient sampling set selection for
  bandlimited graph signals using graph spectral proxies,'' \emph{IEEE Trans.
  Sig. Process.}, vol.~64, no.~14, pp. 3775--3789, Jul. 2016.

\bibitem{BGG14}
B.~Baingana, G.~Mateos, and G.~B. Giannakis, ``Proximal-gradient algorithms for
  tracking cascades over social networks,'' \emph{IEEE J. Sel. Topics Sig.
  Proc.}, vol.~8, no.~4, pp. 563--575, Aug. 2014.

\bibitem{bertsekas1999nonlinear}
D.~Bertsekas, \emph{Nonlinear {P}rogramming}.\hskip 1em plus 0.5em minus
  0.4em\relax Athena Scientific Belmont, 1999.

\bibitem{cai2013inference}
X.~Cai, J.~A. Bazerque, and G.~B. Giannakis, ``Inference of gene regulatory
  networks with sparse structural equation models exploiting genetic
  perturbations,'' \emph{PLoS Comp. Biol.}, vol.~9, no.~5, p. e1003068, May
  2013.

\bibitem{chen2014clustering}
Y.~Chen, A.~Jalali, S.~Sanghavi, and H.~Xu, ``Clustering partially observed
  graphs via convex optimization,'' \emph{J. Mach. Learn. Res.}, vol.~15,
  no.~1, pp. 2213--2238, 2014.

\bibitem{dong2015learning}
X.~Dong, D.~Thanou, P.~Frossard, and P.~Vandergheynst, ``Learning laplacian
  matrix in smooth graph signal representations,'' \emph{IEEE Trans. Sig.
  Process.}, vol.~64, no.~23, pp. 6160--6173, Dec. 2016.

\bibitem{giannakis2016decentralized}
G.~B. Giannakis, Q.~Ling, G.~Mateos, I.~D. Schizas, and H.~Zhu, ``Decentralized
  learning for wireless communications and networking,'' in \emph{Splitting
  Methods in Communication, Imaging, Science, and Engineering}.\hskip 1em plus
  0.5em minus 0.4em\relax Springer, 2016, pp. 461--497.

\bibitem{goldberger1972structural}
A.~S. Goldberger, ``Structural equation methods in the social sciences,''
  \emph{Econometrica}, vol.~40, no.~6, pp. 979--1001, Nov. 1972.

\bibitem{harring2012comparison}
J.~R. Harring, B.~A. Weiss, and J.-C. Hsu, ``A comparison of methods for
  estimating quadratic effects in nonlinear structural equation models.''
  \emph{Psychological Methods}, vol.~17, no.~2, pp. 193--214, Jun. 2012.

\bibitem{ioannidis2016semipar}
V.~N. Ioannidis, A.~N. Nikolakopoulos, and G.~B. Giannakis, ``Semi-parametric
  graph kernel-based reconstruction,'' in \emph{Global Conf. Sig. Inf.
  Process.}, Montreal, Canada, Nov. 2017.

\bibitem{kaplan09}
D.~Kaplan, \emph{Structural Equation Modeling: Foundations and
  Extensions}.\hskip 1em plus 0.5em minus 0.4em\relax Sage, 2009.

\bibitem{kivela2014multilayer}
M.~Kivel{\"a}, A.~Arenas, M.~Barthelemy, J.~P. Gleeson, Y.~Moreno, and M.~A.
  Porter, ``Multilayer networks,'' \emph{Journal of {Complex Networks}},
  vol.~2, no.~3, pp. 203--271, 2014.

\bibitem{kolaczyck2009}
E.~D. Kolaczyk, \emph{Statistical Analysis of Network Data: Methods and
  Models}.\hskip 1em plus 0.5em minus 0.4em\relax Springer New York, 2009.

\bibitem{leskovec2010kronecker}
J.~Leskovec, D.~Chakrabarti, J.~Kleinberg, C.~Faloutsos, and Z.~Ghahramani,
  ``Kronecker graphs: An approach to modeling networks,'' \emph{J. Mach. Learn.
  Res.}, vol.~11, no.~2, pp. 985--1042, Feb. 2010.

\bibitem{marques2016aggregations}
A.~G. Marques, S.~Segarra, G.~Leus, and A.~Ribeiro, ``Sampling of graph signals
  with successive local aggregations,'' \emph{IEEE Trans. Sig. Process.},
  vol.~64, no.~7, pp. 1832--1843, Apr. 2016.

\bibitem{muthen1984general}
B.~Muth{\'e}n, ``A general structural equation model with dichotomous, ordered
  categorical, and continuous latent variable indicators,''
  \emph{Psychometrika}, vol.~49, no.~1, pp. 115--132, Mar. 1984.

\bibitem{narang2013localized}
S.~K. Narang, A.~Gadde, E.~Sanou, and A.~Ortega, ``Localized iterative methods
  for interpolation in graph structured data,'' in \emph{Global Conf. Sig. Inf.
  Process.}, Austin, Texas, 2013, pp. 491--494.

\bibitem{romero2016spacetimekernel}
D.~Romero, V.~N. Ioannidis, and G.~B. Giannakis, ``Kernel-based reconstruction
  of space-time functions on dynamic graphs,'' \emph{IEEE J. Sel. Topics Sig.
  Process.}, vol.~11, no.~6, pp. 1--14, Sep. 2017.

\bibitem{romero2016multikernel}
D.~Romero, M.~Ma, and G.~B. Giannakis, ``Kernel-based reconstruction of graph
  signals,'' \emph{IEEE Trans. Sig. Process.}, vol.~65, no.~3, pp. 764--778,
  Feb. 2017.

\bibitem{segarra2016templates}
S.~Segarra, A.~G. Marques, G.~Mateos, and A.~Ribeiro, ``Network topology
  inference from spectral templates,'' \emph{IEEE Trans.  Sig. and Info.
  Process. over Net.}, vol.~3, no.~3, pp. 467--483, Sep. 2017.

\bibitem{shen2016kernelsvarm}
Y.~Shen, B.~Baingana, and G.~B. Giannakis, ``Nonlinear structural vector
  autoregressive models for inferring effective brain network connectivity,''
  \emph{arXiv preprint arXiv:1610.06551v1}, 2016.

\bibitem{shen2017tensor}
Y.~Shen, B.~Baingana, and G.~B. Giannakis, ``Tensor decompositions for identifying directed graph 
topologies and
  tracking dynamic networks,'' \emph{IEEE Trans. Sig. Process.}, vol.~65,
  no.~14, pp. 4004--4018, July 2017.

\bibitem{shen2017tsp}
Y.~Shen, B.~Baingana, and G.~B. Giannakis, ``Kernel-based structural equation models for topology 
identification
  of directed networks,'' \emph{IEEE Trans. Sig. Process.}, vol.~65, no.~10, pp.
  2503--2516, May 2017.

\bibitem{shuman2013emerging}
D.~I. Shuman, S.~K. Narang, P.~Frossard, A.~Ortega, and P.~Vandergheynst, ``The
  emerging field of signal processing on graphs: Extending high-dimensional
  data analysis to networks and other irregular domains,'' \emph{IEEE Sig.
  Process. Mag.}, vol.~30, no.~3, pp. 83--98, May 2013.

\bibitem{smola2003kernels}
A.~J. Smola and R.~I. Kondor, ``Kernels and regularization on graphs,'' in
  \emph{Learning Theory and Kernel Machines}.\hskip 1em plus 0.5em minus
  0.4em\relax Springer, 2003, pp. 144--158.

\bibitem{thanou2017learning}
D.~Thanou, X.~Dong, D.~Kressner, and P.~Frossard, ``Learning heat diffusion
  graphs,'' \emph{IEEE Trans.  Sig. and Info.
  Process. over Net.}, vol.~3, no.~3, pp. 484--499, 2017.

\bibitem{traganitisnetwork}
P.~A. Traganitis, Y.~Shen, and G.~B. Giannakis, ``Network topology inference
  via elastic net structural equation models,'' in \emph{Proc. European Sig.
  Process. Conf.}, Kos, Greece, Aug. 2017.

\bibitem{tseng2001convergence}
P.~Tseng, ``Convergence of a block coordinate descent method for
  nondifferentiable minimization,'' \emph{J. of Opt. Theo. and Appl.}, vol.
  109, no.~3, pp. 475--494, 2001.

\bibitem{tsitsvero2016uncertainty}
M.~Tsitsvero, S.~Barbarossa, and P.~Di~Lorenzo, ``Signals on graphs:
  Uncertainty principle and sampling,'' \emph{IEEE Trans. Sig. Process.},  vol.~64, no.~18, pp. 
  4845--4860, Sep. 2016.

\end{thebibliography}


==> simulatedtests.tex <==

% parent file: paper.tex

\newcommand{\dlsrstepsize}{\hc{\mu_\text{DLSR}}}
\newcommand{\lmsstepsize}{\hc{\mu_\text{LMS}}}
\newcommand{\dlsrbeta}{\hc{\beta_\text{DLSR}}}
\newcommand{\bandwidth}{\hc{B}}


\cmt{Sec. overview}This section compares the performance of the
proposed schemes with state-of-the-art alternatives and illustrates
some of the trade-offs inherent to time-varying function
reconstruction through real-data experiments.  \cmt{compared
  est.}Unless otherwise stated, the compared estimators include
\begin{myitemize}
\myitem distributed least squares reconstruction
(DLSR)~\cite{wang2015distributed} with step size $\dlsrstepsize$ and
parameter $\dlsrbeta$; \myitem the least mean-square (LMS) algorithm
in~\cite{lorenzo2016lms} with step size $\lmsstepsize$; \myitem
bandlimited instantaneous estimator (BL-IE), which results from
applying~\cite{narang2013localized,tsitsvero2016uncertainty,anis2016proxies}
%gadde2015probabilistic
separately per $\timeind$; \myitem KRR instantaneous estimator
(KRR-IE) reconstruction in \eqref{eq:timeagnostic} with a diffusion
kernel with parameter $\sigma$; \myitem and the proposed KKF
(Algorithms~\ref{algo:rec} and~\ref{algo:kalmanfilter}) with kernel
given by \eqref{eq:kerneltimevarying} for
$\timeconnectionmat\timenot{\timenum}=\timeconnection\bm I$ and
$\spacefullkernelmat\timenot{\timeind}$ a diffusion kernel with
parameter $\sigma$.
\end{myitemize}
DLSR, LMS, and BL-IE also use a bandwidth
parameter~$\bandwidth$.

\cmt{Data set 1: Temperature evolution across contiguous USA} The
first data set comprises hourly temperature measurements at
$\vertexnum=109$ stations across the continental U.S. in
2010~\cite{USATemp}. Temperature reconstruction has been extensively
employed in the literature to analyze the performance of inference
tools over graphs (see
e.g.~\cite{mei2016causal,wang2015distributed,bach2004learning}).%%  and
%% \myitem\cmt{Motivation for reconstruction}is well-motivated by
%% malfunctioning sensors as well as the need for estimating temperature
%% at locations where no sensor has been deployed.
\begin{myitemize}\myitem\cmt{Configuration}\begin{myitemize}
    \myitem\cmt{adjacency}A time-invariant graph was constructed
    following the approach in~\cite{mei2016causal} with 7 nearest
    neighbors, which relies on geographical
    distances.%%  \cmt{Intuition}This approach relies on geographical
    %% distances, which is motivated by the intuitive argument that
    %% geographically close stations tend to measure similar temperature
    %% values.
    \myitem\cmt{signal} Function
    $\signalfun\timevertexnot{\timeind}{\vertexind}$ represents the
    temperature at the $\vertexind$-th  station and
    $\timeind$-th sampling instant. In the first experiment, the
    latter corresponds to the $\timeind$-th hour, whereas for the
    rest, it corresponds to the temperature at 12:00 PM of the
    $\timeind$-th day.
       
  \end{myitemize} 

      \myitem\cmt{Experiment 1:NMSE vs time importance of decomposition
	\ra Fig.~\ref{fig:nmseDecomp}}  

	\begin{figure}
	    \centering
%	    \hspace{-0.3cm}
	    \includegraphics[width=8.5cm]{figs/KFonGSimulations_2218-1}
	  \caption{True temperature and estimates across time at a
            randomly picked unobserved station ($\regpar=10^{-7}$,
            $\sigma=1.8$).}
	    \label{fig:nmseDecomp}
	\end{figure}


      \begin{myitemize}
	\myitem\cmt{goal}Fig.~\ref{fig:realTempTrack} depicts the true
        temperature measured at an unobserved randomly picked station
        over the first 200 hours of 2010 along with its estimates for
        a typical realization of the time-invariant sampling set
        $\sampleset=\sampleset\timenot{\timeind},~\forall\timeind,$
        drawn at random within all sampling sets with $\samplenum=44$
        elements.  \myitem\cmt{Observations}Different from
        instantaneous  alternatives, whose error does not
        decrease with time, KKF is observed to successfully leverage
        time dynamics to track the temperature at the unobserved
        station.  On the other hand, DLSR and LMS are unable to track
        the rapid variations of $\signalfun$ since their design
        assumes slowly changing functions.
      \end{myitemize}
      

\cmt{NMSE def}The next experiments compare the cumulative normalized
mean-square error (NMSE), defined as
  \begin{align*}
    \text{NMSE}(\timeind,\{\sampleset\timenot{\tau}\}_{\tau=1}^\timeind):=\frac{\sum_{\tau=1}^{\timeind}
      ||\samplemat^c\timenot{\tau}(\signalvec\timenot{\tau}
      -\signalestvec\timenot{\tau|\tau})||^2_2}
	 {\sum_{\tau=1}^{\timeind}	 
	   ||\samplemat^c\timenot{\tau}\signalvec
	   \timenot{\tau}||^2_2}
  \end{align*}
  where $\samplemat^c\timenot{\tau}$ is an
  $\vertexnum-\samplenum\timenot{\tau}\times \vertexnum$ matrix
  comprising the rows of $\identitymat_\vertexnum$ whose indices are
  not in $\sampleset\timenot{\timeind}$.






      \myitem\cmt{Experiment 2: error vs. time 
	Fig.~\ref{fig:realTemp} }
      \begin{myitemize}
	\begin{figure}
%	  \begin{minipage}[h]{0.5\linewidth}
	    \centering
%	    \hspace{-0.3cm}
	    \includegraphics[width=8.5cm]{figs/KFonGSimulations_2219-1}
	    
%	    \subcaption{}
	   
%	  \end{minipage}%
	  
	  \caption{NMSE of daily temperature estimates over 2010.
	    ($\regpar=10^{-7}$,
	    $\sigma=1.8$,
	    $\timeconnection =0.01$,
	    $\dlsrstepsize =1.2$,
	    $\dlsrbeta=0.5$,
	    $\lmsstepsize =0.6$).
}
	 \label{fig:realTemp}
	\end{figure}
	%	%
	

	\myitem\cmt{Goal}Fig.~\ref{fig:realTemp} shows the NMSE for
        $\sampleset\timenot{\timeind} = \sampleset,~\forall\timeind$,
        averaged over all possible $\sampleset$ with $\samplenum=44$
        elements.  \myitem\cmt{Observations}It is observed that the
        instantaneous estimators outperform DLSR and LMS, which can
        only cope with slow variations of $\signalfun$. Furthermore,
        the error of KKF is half the error of the nearest alternative,
        demonstrating the importance of exploiting time dynamics.
      \end{myitemize}
      
      \myitem\cmt{Experiment 3:  error vs sampling 
	size\ra Fig.~\ref{fig:realTempIncrSamp}}  
      \begin{myitemize}
	\begin{figure}
%	  \begin{minipage}[h]{0.5\linewidth}
	    \centering
%	    \hspace{-0.3cm}
	    \includegraphics[width=8.5cm]{figs/KFonGSimulations_2216-1}
	    
%	    \subcaption{}
%	  \end{minipage}%
	  
	  \caption{NMSE for increasing sampling size
	  	($\regpar=10^{-7}$,
	  	$\sigma=1.6$,
	  	$\timeconnection =0.01$,
	  	$\dlsrstepsize =1.2$,
	  	$\dlsrbeta=0.5$,
	  	$\lmsstepsize =0.6$).}
	    \label{fig:realTempIncrSamp}
	\end{figure}
	%	%

	\myitem\cmt{Goal}Fig.~\ref{fig:realTempIncrSamp} shows
        the impact of the number of observed vertices $\samplenum$ in
        $\text{NMSE}(\timenum,\{\sampleset\timenot{\timeindaux}\}_{\tau=1}^\timeind)$,
        with $\timenum=365$ days, averaged over all sets
        $\sampleset\timenot{\timeindaux}=\sampleset~\forall\timeindaux$
        with $\samplenum$ elements.  \myitem\cmt{Observations}Observe
        that KKF consistently outperforms all alternatives. Still, the
        advantage of KKF over KRR-IE is more pronounced for small
        $\samplenum$, since in that case exploiting the time dynamics
        is more critical.
      \end{myitemize}

      \myitem\cmt{Experiment 4: error vs offdiag scaling \ra
        Fig.~\ref{fig:paramselection}}
      \begin{myitemize}
	\begin{figure}
	    \centering
	    \includegraphics[width=8.5cm]{figs/KFonGSimulations_2223-1}
	  \caption{NMSE for different kernels vs. scale parameter $
            \timeconnection$ ($\regpar=10^{-7}$).
	    %% \cmt{I could not change the tic positions in 
	    %%   the x axis using Ffigure object meaning add 
	    %%   tics for 1000,10000..}
            }
	    \label{fig:paramselection}
	\end{figure}
	\myitem\cmt{Goal}To illustrate the trade-off between
        reliance on temporal versus spatial information, the next
        experiment analyzes the effects of the scaling parameter $
        \timeconnection$ in the kernel adopted by KRR
        (cf.~\eqref{eq:kerneltimevarying}). A large value of
        $\timeconnection$ leads to an estimator that relies more
        heavily on time dynamics and vice versa.
        Fig.~\ref{fig:paramselection} shows
        $\text{NMSE}(\timenum,\{\sampleset\timenot{\tau}\}_{\tau=1}^\timeind)$,
        with $\timenum=365$ days, averaged over sets
        $\sampleset\timenot\timeind$, which are chosen per $\timeind$
        uniformly at random among all sets of $\samplenum=44$
        elements.  \myitem\cmt{Kernels used}The kernel
        in~\eqref{eq:kerneltimevarying} is adopted with
        $\spacefullkernelmat\timenot{\timeind}$ being the regularized
        Laplacian (KKF-L) or diffusion kernels (KKF-DF) from Table
        \ref{tab:spectralweightfuns}, while
        $\timeconnectionmat\timenot{\timenum}=\timeconnection\bm I$.
        \myitem\cmt{Result}It is observed that there exists an optimum
        value for $\timeconnection$ which leads to the best
        reconstruction performance. This corresponds to the optimal
        trade-off point between reliance on temporal and spatial
        information. Moreover, if $\timeconnection$ is set to its
        optimum value, the impact of the kernel choice is small,
        meaning that a proper exploitation of temporal dynamics also
        reduces the effects of kernel selection; see
        also~\cite{romero2016multikernel}.


%% We observe that the diffusion kernel
%%         achieves improved reconstruction than the regularized
%%         Laplacian. Moreover increasing $\timeconnection$ is beneficial
%%         for reconstruction.  This can be explained from the random
%%         sampling at each time, which suggests that KKF estimates
%%         should rely mainly on the value of the signal at the same
%%         vertix for $\timeind-1$, which in
%%         \eqref{eq:regularizertimevaryingkernel} is controlled by the
%%         value of $\timeconnection$ .  Interestingly for large
%%         $\timeconnection$ NMSE increases, since
%%         $\signalestfun\timevertexnot{\timeind}{\vertexind}$ is almost
%%         the same for all $\timeind$.
	
	
      \end{myitemize}
      %						\myitem\cmt{like rajawat2014}While the NMSPE is 
      %						useful for 
      %						characterizing the average
      %						performance, network operators are also 
      %						interested in the
      %						prediction accuracy over the entire range of 
      %						delay values.
      %						Towards this end, Fig. 7 shows the scatter 
      %						plots of 
      %						predicted
      %						versus	true  for all t and  all vertices or 
      %						only the 
      %						unsampled?
      %						\myitem\cmt{rajawat2014}True and predicted 
      %						delay map for 62 
      %						paths in the Internet2 network
      %						over in interval of 100 minutes. (a) True map. 
      %						(b) Kriging. 
      %						(c) 
      %						Wavelets.
      %						(d) KKF.
      
      

      


\end{myitemize}


\cmt{Data set 2: Economic sectors} The second data set is provided by
the Bureau of Economic Analysis of the U.S.  Department of Commerce
and contains the annual investments between two sectors among
$\vertexnum=58$ economic sectors in the interval 1998-2011, thus
comprising $\timenum=14$
years~\cite{BEconanalysis}.
\begin{myitemize}\myitem\cmt{Configuration}\begin{myitemize}\myitem\cmt{adjacency}Matrix
    $\spaceadjacencymat\timenot{\timeind}$,
    $\timeind=1,\ldots,\timenum$, was constructed by applying the
    procedure in~\cite{marques2015aggregations} to the $\timeind$-th
    year.  DLSR and LMS adopt
    $\spaceadjacencymat=({1}/{\timenum})\sum_{\tau=1}^{\timenum}
    \spaceadjacencymat\timenot{\tau}$ since they cannot handle
    time-varying topologies.  \myitem\cmt{signal} The value
    $\signalfun\timevertexnot{\timeind}{\vertexind}$ corresponds to
    the total production of the $\vertexind$-th sector in year~$\timeind$.
	

	
	%% \myitem\cmt{Motivation for reconstruction} Observing the 
	%% economic activity of some sectors and predicting the output of 
	%% others based on historical data and sectors' relations is 
	%% useful. The government's investment policy can be driven so 
	%% that the desired production is achieved in one sector.
      \end{myitemize} 



      \myitem\cmt{Experiment 1: error
        vs. time~\ref{fig:econnmseacrosstime} }  
      \begin{myitemize}
	\begin{figure}
	    \centering
	    \includegraphics[width=8.5cm]{figs/KFonGSimulations_5232-1}
	  \caption{NMSE for the economic sectors data set
            ($\sigma=4.2$, $\regpar=10^{-4}$, $\dlsrstepsize=1.2$,
            $\dlsrbeta =0.5$, $\lmsstepsize =0.6$).}
	    \label{fig:econnmseacrosstime}
	\end{figure}
	%% \begin{figure}
	%% 	\begin{minipage}[h]{0.5\linewidth}
	%% 		\centering
	%% 		\hspace{-0.3cm}
	%% 		\includegraphics[width=8.5cm]{figs/KFonGSimulations_5332-1}
			
	%% 		\subcaption{}
	%% 		\label{fig:econsecacrostime}
	%% 	\end{minipage}%
		
	%% 	\caption{ Evolution of the 5 most productive 
	%% 		economic sectors. Notice the sharp change 
	%% 		between 2002 and 2003. \acom{Can be removed in the final paper} }
	%% \end{figure}

	%% \begin{figure}
	%%   \begin{minipage}[h]{0.5\linewidth}
	%%     \centering
	%%     \hspace{-0.3cm}
	%%     \includegraphics[width=8.5cm]{figs/KFonGSimulations_5332-1}
	    
	%%     \subcaption{}
	%%     \label{fig:econsecacrostime}
	%%   \end{minipage}%
	  
	%%   \caption{ Evolution of the 5 most productive 
	%%     economic sectors. Notice the sharp change 
	%%     between 2002 and 2003.  }
	%% \end{figure}
	%	%
	
	\myitem\cmt{Goal}The next experiment demonstrates the ability
        of KKF to handle time-varying topologies and its flexibility
        to accommodate prior information about temporal dynamics.
        \myitem\cmt{Y-axis}To this end,
        Fig.~\ref{fig:econnmseacrosstime} plots
        $\text{NMSE}(\timeind,\{\sampleset\timenot{\tau}\}_{\tau=1}^\timeind)$,
        averaged over all sets
        $\sampleset\timenot\timeind=\sampleset,~\forall\timeind,$ with
        $\samplenum=35$ elements.  \myitem\cmt{Kernels}KKF utilizes
        the kernel in~\eqref{eq:kerneltimevarying} with
        $\spacefullkernelmat\timenot\timeind$ a diffusion kernel
        constructed from $\spacelaplacianmat\timenot\timeind$ per
        $\timeind$ and $\timeconnectionmat\timenot{\timeind}=
        \timeconnection\timenot{\timeind}\bm I,~\forall\timeind$, with
        $\timeconnection\timenot{\timeind}=10^{-7}$ for
        ${\timeind=2003}$, and
        $\timeconnection\timenot{\timeind}=0.01$ otherwise. The reason
        for such a small value of $\timeconnection\timenot{2003}$ is a
        rapid change in the investment activity, which calls for
        estimators that rely more heavily on spatial information over
        the time interval 2000-2002. Such a change was caused by the
        stock market crash of 2002-2003 that followed the burst of the
        dot-com bubble.  \myitem\cmt{Observations}Again,
        Fig.~\ref{fig:econnmseacrosstime} showcases the superior
        performance of the proposed KKF, whose error is half the error
        of competing alternatives.


%% KKF estimate achieves improved 
%% 	reconstruction perfomance compared to LMS and DLSR. KKF can 
%% 	incorporate different topologies, whereas LMS and DLSR 
%% 	must use the same topology for all years. NMSE increases for all
%% 	estimates between 2002-2003. The models 
%% 	assume smoothness over time, which is not the case here\cmt{ as one 
%% 	observes at \ref{fig:econsecacrostime}. The most productive 
%% 	economic sectors exhibit abrupt changes in their output.} 
%% 	This information can be captured by the proposed model by 
%% 	accurately tuning $\timeconnection\timenot{\timeind}$ 
%% 	different for each $\timeind$.
%% 	\acom{I can remove the different $\timeconnection$ if you think it is not 
%% 	needed reconstruction does not change much}
      \end{myitemize}
      


{Finally, further experiments were conducted on a data set of
  ECoG signals (see Sec.~\ref{sec:intro}) and the proposed KKF was
  again observed to outperform existing alternatives. Figures and
  details are omitted here due to lack of space, but will be included
  if the paper is accepted. }

%% \acom{--------------------------------------- Decide whether to add.}
%% \end{myitemize}

%% \cmt{Data set 3: Brain} The third data set comprises of brain signal
%% time-series as monitored in an ECoG study in \acom{cite Kolaczyk}.
%% The signal was measured from $\vertexnum=76$ electrodes,
%% implanted into the subject's brain, and sampled 4000 times over 10
%% seconds. The procedure was 
%% executed 8 times. \acom{we have 8 brain signals 8x76x4000 }

%% \begin{myitemize}\myitem\cmt{Configuration}\begin{myitemize}
%% 		\myitem\cmt{adjacency}The topology
%% 		$\spaceadjacencymat$, was provided by the procedure in \acom{Yannings 
%% 		paper https://arxiv.org/pdf/1610.06551v1.pdf add to reference also in 
%% 		introduction has a section describing the dataset}.  
%% 		\myitem\cmt{signal}
%% 		The electric signal
%% 		$\signalfun\timevertexnot{\timeind}{\vertexind}$
%% 		of the $\vertexind$-th electrode at each
%% 		$\timeind$ time sample \acom{every 250 ms} was considered, 
%% 		corresponding to the 1st of the 8 
%% 		executions of the experiment.
		
%% 	\end{myitemize} 
	
	
	
%% 	\myitem\cmt{Experiment 1: error
%% 		vs. time~\ref{fig:brainacrosstime} }  
%% 	\begin{myitemize}
%% 		\begin{figure}
%% 			\centering
%% 			\includegraphics[width=8.5cm]{figs/KFonGSimulations_3219-1}
%% 			\caption{NMSE for the ECoG data set
%% 				($\regpar=10^{-4}$, $\dlsrstepsize=1.2$,
%% 				$\dlsrbeta =0.5$, $\lmsstepsize =0.6$).}
%% 			\label{fig:brainacrosstime}
%% 		\end{figure}
%% 		\myitem\cmt{Goal}This experiment demonstrates the ability of KKF to use
%% 		prior information and reconstruct without an explicit topology.
%% 		\myitem\cmt{Y-axis}To this end,
%% 		Fig.~\ref{fig:brainacrosstime} plots
%% 		\acom{I first normalize the true function}
%% 		\acom{After I train I add to the estimates the means multiply  with
%% 			the stds }
%% 		\acom{I do the same on the initial true function then I compute the 
%% 			error}	
%% 		$\text{NMSE}(\timeind,\{\sampleset\timenot{\tau}\}_{\tau=1}^\timeind)$,
%% 		averaged over all sets
%% 		$\sampleset\timenot\timeind=\sampleset,~\forall\timeind,$ with
%% 		$\samplenum=60$ electrodes considered.
%% 		\myitem\cmt{Kernels}KKF utilizes
%% 		the kernel in~\eqref{eq:kerneltimevarying} with
%% 		$\spacefullkernelmat\timenot\timeind$ a covariance kernel
%% 		constructed as \acom{sample covariance cov function in matlab}
%% 		\acom{the signals used for sample covariance is ecog data of the 2nd
%% 			brain time series of the 8 available}
%% 		$\timeconnectionmat\timenot{\timenum}=\timeconnection\bm 
%% 		I$ where $\timeconnection=1$. 
%% 		\myitem\cmt{Observations}
%% 		Fig.~\ref{fig:brainacrosstime} shows the ability of KKF to capture prior
%% 		information using the covariance kernel and achieving improved 
%% 		performance
		
		
%% 	\end{myitemize}
	
	
\end{myitemize}






